Advancing Conversational Psychotherapy: Integrating Privacy, Dual-Memory, and Domain Expertise with Large Language Models

Mental health has increasingly become a global issue that reveals the limitations of traditional conversational psychotherapy, constrained by location, time, expense, and privacy concerns. In response to these challenges, we introduce SoulSpeak, a Large Language Model (LLM)-enabled chatbot designed to democratize access to psychotherapy. SoulSpeak improves upon the capabilities of standard LLM-enabled chatbots by incorporating a novel dual-memory component that combines short-term and long-term context via Retrieval Augmented Generation (RAG) to offer personalized responses while ensuring the preservation of user privacy and intimacy through a dedicated privacy module. In addition, it leverages a counseling chat dataset of therapist-client interactions and various prompting techniques to align the generated responses with psychotherapeutic methods. We introduce two fine-tuned BERT models to evaluate the system against existing LLMs and human therapists: the Conversational Psychotherapy Preference Model (CPPM) to simulate human preference among responses and another to assess response relevance to user input. CPPM is useful for training and evaluating psychotherapy-focused language models independent from SoulSpeak, helping with the constrained resources available for psychotherapy. Furthermore, the effectiveness of the dual-memory component and the robustness of the privacy module are also examined. Our findings highlight the potential and challenge of enhancing mental health care by offering an alternative that combines the expertise of traditional therapy with the advantages of LLMs, providing a promising way to address the accessibility and personalization gap in current mental health services.

==> section/discussion.tex <==
\section{Conclusion}\label{sec:discussion}

In summary, this paper presents \soulspeak{}, an LLM-enabled conversational agent that provides low-cost mental health therapy. Souspeak is novel in its preservation of privacy, its psychological nuance when answering questions, and most importantly, its ability to remember content from previous user interactions and integrate it in context with a long-term memory module. An extensive evaluation is conducted with a dataset of chats between licensed therapists and their service users, including finetuning two BERT models for simulating preference and encoding text response, to compare responses from therapists and \soulspeak{} of different settings. Experimental results prove the effectiveness of \soulspeak{} as a possible alternative to traditional therapy sessions. In the future, we plan to enrich our prompt designs and design prompts to work better with different therapy topics. In addition, we wish to release \soulspeak{} to the public and receive feedback to improve its performance iteratively. 

==> section/experiments.tex <==
\section{Evaluation}\label{sec:framework}
To evaluate the proposed system's performance, we implement two sets of metrics to test its ability to respond to an individual question without any contextual information and to respond to a question in a series of conversations. 



\subsection{Metric for Context-dependent Response}
We use GPT-4 to generate multiple scripted interaction scenarios for testing the long-term memory component of the Soulspeak agent. The interaction scenario is designed to include specific details about a person mentioned in the initial messages. Then, the user will ask a question related to that person later in the conversation, allowing for a clear test of the long-term memory retrieval capabilities. An example can be found in Table~\ref{table:gpt4}. We collected 16 scripted interaction scenarios in total, covering a wide range of common topics in therapy.

To evaluate performance, we feed past conversations into our memory module while deactivating the short-term memory context window. This approach ensures that the agent exclusively relies on the long-term memory provided by the entity summarizer. Next, the user's query is sent to the agent. Upon receiving the output, it is compared with the baseline response generated by the agent using GPT-3.5 with the long-term memory disabled. Additionally, we assess whether it includes the specific details the user previously mentioned, as summarized in "Key Information" in Table~\ref{table:gpt4}. Quantitatively, we compute the semantic similarity score between GPT-4's answer and both the soulspeak agent and the GPT-3.5 baseline.


==> section/result.tex <==
\section{Performance Analysis}\label{sec:analysis}





The effectiveness of the proposed system is analyzed using the results of the aforementioned evaluation framework. The LLM used in the experiment is OpenAI's GPT-3.5-turbo-1106. 



\begin{table*}[ht]
\centering
\caption{\textbf{Ablation Study of Long-term Memory Module} Average relevance scores computed over 16 GPT-4 generated therapy scenarios.}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Configuration} & \textbf{GPT-4 Therapist Response} & \textbf{Expected Information} \\ \hline
GPT-3.5 Baseline & 0.4089 & 0.3091 \\ \hline
Soulspeak with Long-term Memory & 0.6495 & 0.4911 \\ \hline
\end{tabular}
\label{table:ablation_study}
\end{table*}

\subsection{Privacy module}
We use the model "en\_core\_web\_lg-3.7.1" from the spaCy NLP library as the default model to perform name entity recognition on the user input. Therefore, the effectiveness of our privacy module is heavily dependent on the performance of the spaCy model. We utilized the benchmark dataset available from spaCy's model releases \citet{spacy_en_core_web_lg_3.7.1}, which provides metrics for NER performance. 


The model performs reasonably well with an F-score of 85.43\%, Recall of 85.7\% and Precision of 85.16\%. This performance level suggests that our privacy module is capable of reliably detecting and handling sensitive information, thereby enhancing the privacy and security aspects of the system.

\subsection{Long-term memory module}

The effectiveness of the long-term memory module in Soulspeak is evaluated both qualitatively and quantitatively. The qualitative results, presented in Table~\ref{table:memory_comparison}, highlight the module's capability to retain and utilize key information from previous interactions. Unlike the baseline GPT-3.5 model, Soulspeak adeptly records and retrieves relevant details about the entity "\textit{Derek.}" This functionality enables the agent to incorporate context from past user-therapist interactions effectively, as evidenced by its accurate recall of the user's feelings of being "\textit{dismissed or hesitant to speak up.}" This accuracy has been consistently observed across all 16 therapy scenarios generated by GPT-4, indicating the robustness of the entity store in capturing essential information mentioned by the user.

% \textbf{Quantitative Evaluation Metrics:}
The long-term memory module's performance is quantified using the relevance scores defined in Section~\ref{subsec:relevance}. These scores measure the closeness between Soulspeak's responses and the GPT-4 sample answers, as well as the key information identified in each scenario (examples of "Sample Answer" and "Key Information" are provided in Table~\ref{table:gpt4}). The evaluation results are summarized in Table~\ref{table:ablation_study}. Soulspeak with long-term memory demonstrates a marked improvement over the GPT-3.5 baseline. Its responses show greater alignment with the "ground truth" provided by GPT-4 generated answers and key information summaries in the test cases. Together with the qualitative insights, we conclude that the long-term memory module effectively enriches the agent's responses by integrating useful information from earlier therapy sessions into the current context.
